Describing emotions with acoustic property prompts for speech emotion recognition

Emotions lie on a broad continuum and treating emotions as a discrete number of classes limits the ability of a model to capture the nuances in the continuum. The challenge is how to describe the nuances of emotions and how to enable a model to learn the descriptions. In this work, we devise a method to automatically create a description (or prompt) for a given audio by computing acoustic properties, such as pitch, loudness, speech rate, and articulation rate. We pair a prompt with its corresponding audio using 5 different emotion datasets. We trained a neural network model using these audio-text pairs. Then, we evaluate the model using one more dataset. We investigate how the model can learn to associate the audio with the descriptions, resulting in performance improvement of Speech Emotion Recognition and Speech Audio Retrieval. We expect our findings to motivate research describing the broad continuum of emotion

==> latexfiles/background.tex <==
% ## MOST recent work on emotion 

% ## Work using both audio and audio description for other tasks 

% ## Work on emotion using other modalities - not necessarily speech and text. 

\ben{I would remove this section for the sake of having enough space for results and briefly describe a bit of the emotion datasets like the slide you have we number of classes, classes name, number of files, etc.}
In computer vision domain, there has been work which uses natural language descriptions of images and images together in a deep learning framework. 
For example, CLIP \cite{radford2021learning} is trained on image-text pairs where these pairs are collected from the internet. The learned model associates image captions with the images. Applying the learned model on various downstream tasks like zero-shot image classification and text retrieval, SoTA performance is achieved on many of them. 

A similar approach has recently been applied to the audio-text pairs in CLAP [CITE]. This model is trained on audio captioning datasets where descriptions for each audio is already present. 
AudioClip \cite{guzhov2022audioclip} is an extension of CLIP, where three modalities are used, audio in addition to image and text. This model is trained on AudioSet \cite{gemmeke2017audio} (contains images, audio and text) where the labels of the audio are used as the textual descriptions. UrbanSound8k \cite{salamon2014dataset} and ESC50 \cite{piczak2015esc} are used to train the audio and text models. 
SimEmotion \cite{deng2022simemotion} performs image emotion recognition, in a similar fashion to CLIP. The textual descriptions for the images are made by extracting emotion and entity level information. The entities in the images are recognized using the Detectron2 library and labelled emotion for the images are expanded using the Plutchik chart. 


==> latexfiles/experiments.tex <==
% \vspace{-0.05cm}
% \subsection{Evaluation Setup}
% We evaluate the model for and under various settings. \\

% \noindent \textbf{Prompt Analysis}: 
% \vspace{-0.1in}
\subsection{Prompt Analysis}
\vspace{-0.05in}
To evaluate which of the proposed acoustic prompts are better [and to see if any of them are better than the class label]. We apply the trained model on emotion classification in a supervised classification setting. The model is trained 6 different times, where each time the description associated with the emotion audios are different. Among the 6, 1 is using the class label alone, 4 are using the acoustic prompts as described in Section 4, and 1 is using the prompt augmentation - combines all the acoustic prompts. 

\vspace{-0.15in}
\subsection{Emotion Classification}
[Why are we doing this experiment]
How using these prompts could help in emotion classification. We have one zero-shot like setup (where we leave one dataset out for testing). Then then we pre-trained model from previous setup and finetune it on the left-out dataset. 

% \subsection{Out of Domain Classification}
\vspace{-0.1in}
\subsubsection{Leave one out}
\vspace{-0.1in}
[Why are we doing this exp]
1. How well the model generalizes to a new dataset. We want to see how a model trained on predefined set of classes generalizes to the same or different classes in a new dataset. 
[Define mismatch][distributional shift]
To perform mismatch emotion classification, out of the 6 emotion datasets, we leave one out for testing and train the model on the other 5 emotion datasets. In case where Ravdess is the testing dataset, `calm' class is not represented in any of the other 5 emotion datasets and could be considered zero shot classification result. 
In case of Crema-d, all the emotion classes are represented in the training classes. 
% There may or may not be an overlap of the emotion classes between the training and testing datasets. For example, when testing on Ravdess, 

\vspace{-0.15in}
\subsubsection{Finetune}
\vspace{-0.1in}
[Why are we doing this exp]
We want to see how using the acoustic prompts at pretraining stage would benefit the classification. 
% \vspace{-0.05in}
We perform supervised classification on the testing subsets of 2 emotion datasets. Once the model is trained on 5 emotion datasets leaving one specific dataset out. The model then acts as a feature extractor and an additional 3 fully connected layers are trained on top using the training folds of the left out dataset. 
% ELABORATE ON THE PARAMETERS

\vspace{-0.15in}
\subsection{Emotion Audio Retrieval}
\vspace{-0.1in}
In order to access whether the trained model learns the associations between the acoustic prompts and the respective acoustic properties, we perform audio retrieval on the emotion datasets. We make queries similarly to the prompts as described in Section 4. An example of query is `high male pitch anger'.
For a given query, the model outputs top $K$ audios whose audio embeddings have highest cosine similarity to the text embedding of the query. For the top $K$ audios, since we know the true acoustic prompts, we can evaluate how good the model's outputs is w.r.t the query. 
% ## Retrieval results 

==> latexfiles/result_discussion.tex <==
\vspace{-0.1cm}
\begin{table*}[tbh!]
\caption{Accuracy achieved when the model is trained under different settings and tested on the left out dataset (shown in the  col 2,3) and when finetuned on the dataset (shown in the col 4,5). 4D refers to the 4 audio captioning datasets used in original CLAP model. ED refer to Emotion Datasets.}
    \centering
    \begin{tabular}{lcc|cc}
         \toprule
         & \multicolumn{2}{c}{Leave one out dataset} & \multicolumn{2}{c}{Finetune}  \\
         \toprule
         Training dataset & Crema-d & Ravdess & Crema-d & Ravdess \\
         \midrule
         Random & 16.67 & 12.50 & & \\
         4D & 17.85 &	15.99 &	67.29	& 68.50 \\
        5 ED - \textit{class label} & 	35.22&	22.88 & x & x \\
        4D + [5 ED - \textit{class label}] &	34.68 &	38.46  &	72.86&	68.69\\
        4D + [5 ED - \textit{prompt augmentation}] &	33.00 &	27.88 &	72.56	& 72.46\\
        SoTA & & & 75.20 & 80.21 \\
        \bottomrule
        \vspace{-1cm}
    \end{tabular}
    \label{tab:ood_supervised_results}
\end{table*}


\vspace{-0.1in}
\subsection{Prompt Analysis}
\vspace{-0.05in}
\begin{figure}[tbh!]
  \centering
  \vspace{-0.3cm}
%   \includegraphics[width=0.7\linewidth,height=0.3\linewidth]{images/prompt_cremad}
%   \includegraphics[width=0.45\linewidth,height=0.4\linewidth]{images/prompt_ravdess}
  \includesvg[width=0.45\linewidth,height=0.6\linewidth]{images/prompt_cremad}
  \includesvg[width=0.45\linewidth,height=0.6\linewidth]{images/prompt_ravdess}
  \caption{Accuracy achieved using different prompts on CREMA-D (left) and RAVDESS (right). A=class-label, B=pitch-prompt, C=intensity-prompt, D=speech-rate-prompt, E=articulation-rate-prompt, F=prompt-augmentation.}
    \label{fig:prompt_analysis}
          \vspace{-0.1in}
\end{figure}
For prompt analysis, we train the model on 4 audio captioning datasets and 1 emotion dataset. Figure \ref{fig:prompt_analysis} shows the performance achieved when the model is trained on the training set and tested on the testing sets of Ravdess and Crema-d respectively.
We observe that among the 4 acoustic prompts, pitch prompt gives the best performance. Next best performance is achieved by the intensity prompt. This can be observed in both Ravdess and Crema-d. On Crema-d, articulation rate prompt performs better than speech rate prompt but the reverse is observed in Ravdess. [WHY]   
Secondly, we observe that overall prompt augmentation is giving the best performance in both datasets. This is encouraging to see due and it validates the original hypothesis that using acoustic prompts would help the emotion classification. 
% ADD ABOUT THE CLASS RPOMPT
\vspace{-0.3cm}
\subsection{Emotion Classification}
\vspace{-0.1in}
\subsubsection{Leave one out}
\vspace{-0.05in}
% ## ood results 
We perform 4 experiments, shown in columns 2,3 of Table~\ref{tab:ood_supervised_results}. Firstly, we train the model on only 4 audio captioning datasets (4D) and evaluate on Ravdess and Crema-d. This is zero shot classification since none of the emotion classes are represented in the training datasets. We achieve 17.85\% accuracy on Crema-d and 15.99\% on Ravdess. 
Secondly we train on only 5 ED, leaving one dataset out. When trained on all 5, excluding Crema-d, we achieve 35.22\% on Crema-d. When trained on all 5 ED except for Ravdess and tested on it, we achieve 22.88\%.  
Thirdly we train the model on all 4D and 5ED, leaving one out. We achieve 34.68\% on Crema-d, which is a slight degradation from the second experiment.
Done similarly on Ravdess, we see a lot of improvement, boosting performance to 38.46\%.
Lastly, this experiment setting is similar to the third one except that for the ED, we perform prompt augmentation. We observe that it slightly degrades performance on both datasets. For Crema-d the performance drops to 33\% and for Ravdess to 27.88\%. 

There are two learnings from these results. Firstly adding ED is helping the performance on a new emotion dataset. Secondly, prompt augmentation's results are similar to the results obtained when trained using only the class label. This is in contrast to what was observed in Section 6.1, and we hypothesize that this is because of the amount of data. When the training data size is large, like in the current experiment, the benefit from using the acoustic prompts decrease. 

[In 6.1, we do not have mismatch condition, but there there is a mismatch condition. The mismatch condition is quite strong and results in this drop in performance. ]
[However we do observe improvement when we include dataset in the training in next section. ]

\vspace{-0.2in}
\subsubsection{Finetune}
\vspace{-0.05in}
[Takeway] 
Fine tuning show that adding prompt augmentation kinda of improves performance. In ravdess, we improved performance by absolute 4\%. In crema-d the performance did not improve, but the accuracy is about the same as when the prompt augmentation is not used. 

The results for supervised classification are shown in columns 4,5 of Table~\ref{tab:ood_supervised_results}. 
Firstly when the model is trained on only 4D and finetuned on Crema-d, we achieve 67.29\%, when done similarly for Ravdess we achieve 68.5\%.
Secondly when trained on 4D and 5ED and finetuned on the chosen datasets, we observe performance improvement in both the datasets; 72.8\% in Crema-d and 68.69\% in Ravdess.
Thirdly when we train a model on 4D and 5ED including prompt augmentation, we observe a slight decrease in performance for Crema-d. The performance improves for Ravdess to 72.46\%. [WHY]
We perform 5 fold cross validation for both datasets. Note that we dont perform the experiment where the model is only trained on only 5ED due to our observation in section 6.2.1 where 4D+5ED lead to better performance than 5ED alone. 

% \begin{table}[]
%     \caption{Accuracy achieved when the model is trained under different settings and tested on the left out dataset.}
%     \centering
%     \begin{tabular}{lcc}
%     \toprule
%         &  \multicolumn{2}{c}{Leave one dataset out} \\
%         % \hline
%         Training Dataset & Crema-d & RAVDESS  \\
%         \midrule
%         Random & 16.67 & 12.50 \\
%         4D & 17.85 &	15.99 \\
%         5 ED {class label} & 	35.22&	22.88\\
%         4D + [5 ED {class label}] &	34.68 &	38.46\\
%         4D + [5 ED + prompt augmentation] &	33.00 &	27.88\\
%          \bottomrule
%     \end{tabular}
%     \label{tab:zero_shot_results}
% \end{table}
% % ## Supervised classification result 
% \begin{table}[]
%     \caption{Accuracy achieved when the model is trained under different settings and then finetuned with on a specific training folds of the dataset.}
%     \centering
%     \begin{tabular}{lcc}
%     \toprule
%     %     &  \multicolumn{2}{c}{Dataset} \\
%     %     % \hline
%         Training Dataset & Crema-d & RAVDESS  \\
%     \midrule
%         SoTA & 75.20 & 80.21 \\
%         4D  &	67.29	& 68.50 \\
% 4D + [5 ED {class label}] &	72.86&	68.69\\
% 4D + [5 ED + 5 prompt augmentation]  &	72.56	& 72.46 \\ 
% \bottomrule
%     \end{tabular}
%     \label{tab:supervised_results}
% \end{table}



% \vspace{-0.35in}
\vspace{-0.7cm}
\subsection{Audio Retrieval}
\vspace{-0.05in}
[Where do we use audio retrieval.][We want to know if the acoustic property are connected and this retrieval allows to evaluate the emotions in the continuum] [How the retrieval numbers compare to audio retrieval precision numbers. cite the paper]
Figure~\ref{fig:retrieval} shows the results of audio retrieval. We calculate precision@$K$ for each acoustic prompt shown on the x-axis. 
% Precision@$K$ is the proportion of relevant items that come up in top $K$ items. 
[Takeaway at the top here]. [This suggests that we can introduce more elaborate descriptions, and be to retrieve audios including the descriptions.]
We evaluate using 3 different models, one trained on 4D, one trained with an additional 5 ED, and the third with an additional of prompt augmentation. We observe that the model trained on all datasets, and using prompt augmentation performs the best in all cases. The takeaway here is that our model is able to retrieve audio significantly better when trained using prompt augmentation. 

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\linewidth,height=0.5\linewidth]{images/retrieval.png}
    \caption{Precision@K achieved when the trained model under different settings is used for the audio retrieval task.}
    \label{fig:retrieval}
\end{figure}

==> latexfiles/result_table.tex <==
% ## Acoustic prompts results 
\begin{table}[]
    \centering
    \begin{tabular}{c|c|c}
         &  Crema-d & RAVDESS\\
        Random & 16.67 & 12.50 \\
        {class} & 69.56 & 66.90 \\
        pitch prompt {class} & 67.80 & 69.42 \\
        intensity prompt {class} & 62.10 & 51.92 \\
        speech rate prompt {class} & 58.60 & 49.23 \\
        articulation prompt {class} & 61.22 & 39.23 \\
        Prompt augmentation & 71.91 & 70.70 \\
    \end{tabular}
    \caption{The following table shows how the accuracy changes based on the acoustic property prompts used. We can observe that the pitch prompt is performing the best among all the acoustic prompts. Overall prompt augmentation performs the best.}
    \label{tab:acoustic_property_prompt_analysis}
\end{table}





\begin{table}[]
    \caption{Accuracy achieved when the model is trained under different settings and tested on the left out dataset.}
    \centering
    \begin{tabular}{lcc}
    \toprule
        &  \multicolumn{2}{c}{Leave one dataset out} \\
        % \hline
        Training Dataset & Crema-d & RAVDESS  \\
        \midrule
        Random & 16.67 & 12.50 \\
        4D & 17.85 &	15.99 \\
        5 ED {class label} & 	35.22&	22.88\\
        4D + [5 ED {class label}] &	34.68 &	38.46\\
        4D + [5 ED + prompt augmentation] &	33.00 &	27.88\\
         \bottomrule
    \end{tabular}
    \label{tab:zero_shot_results}
\end{table}
% ## Supervised classification result 
\begin{table}[]
    \caption{Accuracy achieved when the model is trained under different settings and then finetuned with on a specific training folds of the dataset.}
    \centering
    \begin{tabular}{lcc}
    \toprule
    %     &  \multicolumn{2}{c}{Dataset} \\
    %     % \hline
        Training Dataset & Crema-d & RAVDESS  \\
    \midrule
        SoTA & 75.20 & 80.21 \\
        4D  &	67.29	& 68.50 \\
4D + [5 ED {class label}] &	72.86&	68.69\\
4D + [5 ED + 5 prompt augmentation]  &	72.56	& 72.46 \\ 
\bottomrule
    \end{tabular}
    \label{tab:supervised_results}
\end{table}

\begin{table}[]
\footnotesize
\caption{Details of the 6 emotion datasets used in the work.}
    \centering
    \begin{tabular}{lcccl}
    \toprule
        % Dataset &\#Audios&Avg. Dur.&Classes&Emotion Classes\\
        Dataset &Audio&Dur.&\#Class&Emotions\\
    \midrule
        \multirow{2}{}{CMU-MOSEI\cite{zadeh2018multimodal}} & \multirow{2}{}{23K} & \multirow{2}{}{7.3s} & \multirow{2}{}{9} & ang, exc, fear, sad, frus, \\ 
        & & & & surprise, hap, disappointed, neu \\
        \hline
        \multirow{2}{}{IEMOCAP\cite{busso2008iemocap}} & \multirow{2}{}{20K} & \multirow{2}{}{4.4s} & \multirow{2}{}{9} & hap, fear, sad,  surprise, excite, \\ 
        & & & & ang, neu, disappointed, frus \\
        \hline
        \multirow{2}{}{MELD\cite{poria2018meld}} & \multirow{2}{}{10K} & \multirow{2}{}{3.6s} & \multirow{2}{}{7} & neu, surprise, fear, sad, \\ 
        & & & & joy, disgust, ang \\
        \hline
        \multirow{2}{}{CREMA-D\cite{cao2014crema}} & \multirow{2}{}{7K} & \multirow{2}{}{5.0s} & \multirow{2}{}{6} & ang, disappointed, fear, hap, \\
        & & & & neu, sad \\
        \hline
        \multirow{2}{}{RAVDESS\cite{livingstone2018ryerson}} & \multirow{2}{}{2.5K} & \multirow{2}{}{5.0s}& \multirow{2}{}{8} & neu, calm, hap, sad, \\ 
        & & & & ang, fear, disgust, surprise \\
        \hline
        CMU-MOSI\cite{zadeh2018multimodal} & 2.2K & 4.2s & 3 & neu, positive, negative \\
    \bottomrule
    \end{tabular}
    \label{tab:emotion_dataset}
\end{table}
